Setting the Trap: Capturing and Defeating Backdoors in Pretrained Language Models through Honeypots

In the field of natural language processing, the prevalent approach involves fine-tuning pretrained language models (PLMs) using local samples. Recent research has exposed the susceptibility of PLMs to backdoor attacks, wherein the adversaries can embed malicious prediction behaviors by manipulating a few training samples. In this study, our objective is to develop a backdoor-resistant tuning procedure that yields a backdoor-free model, no matter whether the fine-tuning dataset contains poisoned samples. To this end, we propose and integrate a honeypot module into the original PLM, specifically designed to absorb backdoor information exclusively. Our design is motivated by the observation that lower-layer representations in PLMs carry sufficient backdoor features while carrying minimal information about the original tasks. Consequently, we can impose penalties on the information acquired by the honeypot module to inhibit backdoor creation during the fine-tuning process of the stem network. Comprehensive experiments conducted on benchmark datasets substantiate the effectiveness and robustness of our defensive strategy. Notably, these results indicate a substantial reduction in the attack success rate ranging from 10\% to 40\% when compared to prior state-of-the-art methods.

==> methods.tex <==
\section{Proposed Method}
\label{sec: proposed method}

Our defense strategy originates from the observations in Section~\ref{sec: preliminary results}, which indicate that poisoned samples frequently involve the injection of words, sentences, or syntactic structures that are effectively identified by lower-layer features in PLMs. As a result, we can develop a honeypot classifier specifically designed to capture the backdoor function. As illustrated in Figure~\ref{fig:pipeline}, our proposed algorithm concurrently trains a pair of classifiers $(f_H, f_T)$ by (a) purposefully training a honeypot classifier $f_H$ to be backdoored and (b) training a task classifier $f_T$ that concentrates on the original task. The honeypot classifier consists of one transformer layer topped with a fully connected layer that exclusively relies on lower-layer features of PLMs to learn the backdoor function. The trainable parameter of the honeypot is denoted as $\theta_{T}$. To further accelerate the backdoor learning process, we apply generalized cross-entropy loss \cite{zhang2018generalized, du2021fairness} to augment the backdoor learning:
\begin{equation}
\mathcal{L}_{GCE}(f(x; \theta_H),y) = \frac{1 - f_y(x; \theta_H)^q}{q},
\label{eq:GCE}
\end{equation}
where $f_y(x; \theta_H)$ is the output probability assigned to the ground truth label $y$. The hyper-parameter $q \in (0, 1]$ controls the degree of bias amplification. As $\lim_{q\rightarrow0} \frac{1 - f_y(x; \theta)^q}{q}= -\log f_y(x; \theta)$, which is equivalent to the standard cross-entropy loss. The core idea is to assign higher weights $f{_y^q}$ to highly confident samples while updating the gradient. 

\begin{equation}
    \frac{\partial GCE(p, y)}{ \partial \theta_H} = f_y^q(x; \theta_H)\cdot\frac{\partial CE(p, y)}{ \partial \theta_H}
\end{equation}

Consequently, the GCE loss encourages a model to focus on the ``easier'' samples, the majority of which are poisoned samples when using the lower layer representations, in contrast to a network trained with CE loss.

Concurrently, we train a task classifier whose primary objective is to learn the original task while avoiding the acquisition of the backdoor function. To achieve this goal, we propose employing a weighted cross-entropy loss ($\mathcal{L}_{WCE}$) specifically designed for this purpose. The WCE loss is expressed as follows:

\begin{equation}
% \begin{array}{cl}
    \mathcal{L}_{WCE}(f_H(x), y) = \sigma(W(x) - c) \cdot \mathcal{L}_{CE}(f_H(x),y),
% \end{array}
\end{equation}
\vspace{-1em}
\begin{equation}
% \begin{array}{cl}
W(x) = \mathcal{L}_{CE}(f_H(x), y)\cdot\frac{|\mathcal{L}_{CE}(f_H(x), y) - \mathcal{L}_{CE}(f_T(x), y)|}{ \mathcal{L}_{CE}(f_T(x), y)},
% \end{array}
\end{equation}

% \begin{equation}
% % \begin{array}{cl}
%     \mathcal{L}_{WCE}(f_T(x), y) = \text{Sign}(W(x) - c) \cdot \mathcal{L}_{CE}(f_T(x),y),~~~~\text{where}
% % \end{array}
% \end{equation}
% \vspace{-1em}
% \begin{equation}
% \begin{array}{cl}
% W(x) = \mathcal{L}_{CE}(f_H(x), y),
% % W(x) = \mathcal{L}_{CE}(f_H(x), y)\cdot\frac{|\mathcal{L}_{CE}(f_H(x), y) - \mathcal{L}_{CE}(f_T(x), y)|}{ \mathcal{L}_{CE}(f_T(x), y)},
% % \end{array}
% \end{equation}
In this formulation, $f_H(x)$ and $f_T(x)$ represent the softmax outputs of the honeypot and task classifiers, while $\mathcal{L}_{CE}$ denotes the standard cross-entropy loss. $\sigma(\cdot)$ denotes the sigmoid function. $W(x)$ signifies the loss weight for sample $x$. This weight is employed to impose penalties on the information obtained by the honeypot module, thereby inhibiting backdoor formation during the tuning process of the PLM task classifier. In our design, $W(x)$ comprises two parts: the first part is the loss of the honeypot module $f_H$, and the second part calculates the relative loss difference between $f_H$ and $f_T$.

We elaborate on how the proposed WCE loss functions. After completing the warmup stage, the CE loss value of poisoned samples in $f_H$ is already significantly lower than that of clean samples, whereas both sample losses are high in $f_T$ since the PLM is untrained. Consequently, $W(x)$ assigns a lower training weight to poisoned samples. During the subsequent training process, as $W(x)$ is higher for clean samples, the CE loss of clean samples in $f_T$ decreases more rapidly than that of poisoned samples, further amplifying the second part of $W(x)$ for clean samples. This positive feedback mechanism ensures that the $W(x)$ for poisoned samples remains significantly lower than for clean samples throughout the entire training process of $f_T$. To prevent loss weight values from becoming too large, we normalize $W(x)$ by dividing it by a Sigmoid function with an offset value $c$. Any $W(x)$ value smaller than $c$ quickly becomes 0, and any value higher than $c$ tends to be 1. This normalization process ensures that $W(x)$ lies within the interval of $(0, 1]$. For our experiments, we set $c$ to 0.1 and designate one epoch as the warmup duration.


